Bayesian Prediction-Powered Inference

Prediction-powered inference (PPI) is a method that improves statistical estimates based on limited human-labeled data. Specifically, PPI methods provide tighter confidence intervals by combining small amounts of human-labeled data with larger amounts of data labeled by a reasonably accurate, but potentially biased, automatic system. We propose a framework for PPI based on Bayesian inference that allows researchers to develop new task-appropriate PPI methods easily. Exploiting the ease with which we can design new metrics, we propose improved PPI methods for several importantcases, such as autoraters that give discrete responses (e.g., prompted LLM ``judges'') and autoraters with scores that have a non-linear relationship to human scores.

==> sections/cuts.tex <==
As an example, the difference estimate can be defined as
\begin{eqnarray*}
\hat{\mu}^{N}_{f(x)} & = & \mean{f(x)}{x}{\twid{S}_N} \\
\hat{\mu}^{n}_{y-f(x)} & = & \mean{y - f(x)}{(x,y)}{S_n} \\
g(S_n, \twid{S}_N) & = & \hat{\mu}^{N}_{f(x)} + \hat{\mu}^{n}_{y-f(x)}
\end{eqnarray*}

In general, we will assume there is a statistic, the \emph{target estimand}, we want to measure in expectation.  For the difference estimate this is
\[  e(S_n,\twid{S}_N, f) \equiv \mean{y}{(x,y)}{S_n}
\]
In each method described below, we will introduce a second statistic, the \emph{proxy estimand}, that has the same expectation as $g$ but lower variance. For the difference estimate the proxy estimand is
\[  g(S_n,\twid{S}_N, f) \equiv  \hat{\mu}_{f(x)} + \hat{\mu}_{y-f(x)}
\]
We must verify analytically that $\expect{g}=\expect{e}$, but will measure variance experimentally.  This is easy to do, since confidence intervals on $g$ can be computed automatically using Monte Carlo integration. (For details and an example of doing this, see Appendix~\ref{sec:python}.) 


-----




PPI is useful and quite general, being based on theories of convex optimization, but it can be difficult to map specific use-cases into PPI. Here we advocate for methods that require only designing a \textit{statistic} which is a function of several \textit{estimates}, and then computing confidence intervals over this statistic.  For the task of Figure~\ref{fig:h100-vs-ar-5000}, we would like to design a statistic that equals $p(H)$ in expectation, but which has a tighter confidence interval.

Bootstrap:

Assume a statistic $g(S_n)$ computed on a sample $S$.

Given sample $S$, create $B$ \emph{bootstrap replicates}
$S^1, \ldots, S^B$ and then compute $g'^1=g(S^1), \ldots, g'^B=g(S^B)$.
Sort these low to high to form a vector $\overline{g'}$, which is an empirical sample of $g(S'|S_n)$.  Given $\alpha$, the lower limit $\ell_g$ of a confidence interval for $1-\alpha$ is found by dropping the lowest $B \alpha/2$ elements of $\overline{g'}$ and taking the lowest remaining value as $\ell_g$,  and the upper limit by dropping the highest $B \alpha/2$ elements and taking the highest remaining value.

\wc{robustness/guarantees}

\wc{relative cost, robustness}

\wc{for Monte Carlo integration}

-----

The \emph{difference estimator} is discussed in more detail below in Sec~\ref{sec:diff-est}: briefly, it is a way of obtaining a tighter confidence interval for an estimate of the mean of some value $y$, if one is given access to a small sample with true values of $y$
and a larger sample of approximate values of $y$.

----



----



We can thus estimate $p(AR=1)$ accurately since we can run the autorater on large sample (above, $n=5000$).  Also note that if the autorater is good, then $p(H=1|AR=1)$ should be close to one, and $(1-p)$ is small and we can also estimate this well, and likewise $p(H=1|AR=0)$ should be close to zero and also can be estimated well.  For this task, we thus use the three estimates
\begin{eqnarray*} 
\hat\theta_{AR=1}  & \mbox{estimated from 5000 auto-rated examples} \\
\hat\theta_{H=1|AR=1} & \mbox{estimated from 100 dual-labeled examples} \\
\hat\theta_{H=1|AR=0} & \mbox{estimated from 100 dual-labeled examples} \\
\end{eqnarray*}
Letting $\boldsymbol{\theta}$ denote $\langle \hat\theta_{AR=1}, \hat\theta_{H=1|AR=1}, \hat\theta_{H=1|AR=0} \rangle$ 
we define the statistic $s(\boldsymbol{\theta})$ as
\[
s(\boldsymbol{\theta}) \equiv
    \hat\theta_{H=1|AR=1} \cdot \hat\theta_{AR=1} + 
    \hat\theta_{H=1|AR=0} \cdot (1 - \hat\theta_{AR=1})
\]
Since $s(\boldsymbol{\theta})$ is just a definition of $p(H=1)$ using the chain rule and $p(AR)$, it is an unbiased estimator for $p(H=1)$, but for strong autorater AR, $s$ will have a small confidence interval.  

What remains is the question of how to \emph{compute} a confidence interval for $s(\boldsymbol{\theta})$, of more generally any statistic based on estimates.
Below we describe below two methods doing this. One is based on the bootstrap, a frequentist non-parametric approach, and one is based on \emph{parametric bootstrap}, which also has a Bayesian justification.

Our hope is that simple approaches to designing and implementing auto-rater assisted statistical tests will unlock novel approaches to making use of autoraters for evaluation in statistically justified ways.  To support this, we present a series of case studies showing how autorater-assisted statistical tests can be designed and empirically verified.
